An Inverse Problem with Partial Neumann Data and $L^{n/2}$ Potentials

We consider a partial data inverse problem with unbounded potentials. Rather than rely on functional analytic arguments or Carleman estimates, we construct an explicit Green's function with which we construct complex geometric optics (CGO) solutions and show unique determinability of potentials in $L^{n/2}$ for the Schr\"odinger equation with partial Neumann data.

==> overviewflat.tex <==
\section{Intro/Overview for flat case}

%\abovedisplayskip=4pt plus 2pt minus 3pt
%\abovedisplayshortskip=4pt plus 2pt minus 3pt
%\belowdisplayskip=4pt plus 2pt minus 3pt
%\belowdisplayshortskip=4pt plus 2pt minus 3pt

In the flat case, we have that the symbol of $h^2\Delta_\phi$ is given by
\[
\sigma(h^2\Delta_\phi) = \xi_n^2 -2i\xi_n - (1-\abs{\xi'}^2) = -(i\xi_n+f_-(\xi'))(i\xi_n+f_+(\xi')) + a_0\,,
\]
where 
\[
f_\pm = 1\pm(1-\rho_0(\xi'))\abs{\xi'} \in S^1_1(\RR^{n-1})\,, a_0 = \abs{\xi'}^2(1-(1-\rho_0(\xi'))^2)\in S^2_1(\RR^{n-1})\,. 
\]
Here, $\rho_0 \in C_c^\infty(\RR^{n-1})$ is chosen so that $\rho_0 \equiv 1$ on $\abs{\xi'}^2 \leq c$ and $\supp{\rho_0}\Subset \{\abs{\xi'}^2 \leq c'\}$. Furthermore, we have some $\rho \in C_c^\infty(\RR^{n-1})$ so that $\rho \equiv 1$ when $\abs{\xi'}^2 \leq c'$ and $\supp{\rho} \Subset \{\abs{\xi'}^2 \leq 1\}$, for $0<c<c'<1$, where we may, for example, take $c=1/16$ and $c'=1/4$.

Quantizing the symbols in our decomposition, we get that
\[
h^2\Delta_\phi = QJ + A_0 = -(B+F_-)(B+F_+) + A_0\,,
\]
where $A_0 = \mathrm{Op}_h(a_0)$, $F_\pm = \mathrm{Op}_h(f_\pm)$, $B = \mathrm{Op}_h(i\xi_n) = h\del_{x_n}$ and $J = B+F_+$ and $Q = -(B+F_-)$.

Let $\tau \colon W^{l,r}(\RR^n) \to L^r(\RR^{n-1})$ be the trace onto the hyperplane $x_n = 0$ for $l \geq 1$ and $1<r<\infty$. 
%\marginnote{I think this may even be defined as $\tau \colon W^{s-l,l,r} \to W^{s,0,r}, s\in\RR,l\geq 1$ since we are working with the flat case, but I don't think we'll need this distinction.}

Furthermore, we let $\mathcal{E} \colon W^{l,r}(\RR^{n-1}) \to C^\infty_c(\RR; W^{l,r}(\RR^{n-1}))$ be the extension of a function, so that the image of a function under $\mathcal{E}$ is constant with respect to $x_n$ for $\abs{x_n}<1$ and is smoothly cut off to zero for larger $\abs{x_n}$.

Let $f\in L^{\mathfrak{f}}(\RR^{n-1})$ be any function.\marginnote{Since I have no clue yet what kind of $L^r$ space $f$ will be in, I'll denote it by $\mathfrak{f}$ and hopefully will figure it out later.}
